StackRAG Agent: Improving Developer Answers with Retrieval-Augmented Generation

Developers spend much time finding information that is relevant to their questions. Stack Overflow has been the leading resource, and with the advent of Large Language Models (LLMs), generative models such as ChatGPT are used frequently. However, there is a catch in using each one separately. Searching for answers is time-consuming and tedious, as shown by the many tools developed by researchers to address this issue. On the other, using LLMs is not reliable, as they might produce irrelevant or unreliable answers (i.e., hallucination). In this work, we present StackRAG, a retrieval-augmented Multiagent generation tool based on LLMs that combines the two worlds: aggregating the knowledge from SO to enhance the reliability of the generated answers. Initial evaluations show that the generated answers are correct, accurate, relevant, and useful.

==> Evaluation-OLD.tex <==
\section{Evaluation}

To evaluate the performance of StackRAG, we conducted a survey among \FHF{XX numbers of???} developers from different positions, including Machine Learning Engineers, NLP engineers, as well as Back-end and Front-end developers. These developers often use ChatGPT to find answers to their development-related questions.
\FHF{The developers have ???? years of experience working in industry.}
We used two different approaches. Firstly, we gave the developers access to the tool so that they can use it throughout a whole day in their daily tasks. 
Afterwards, we asked developers to evaluate the generated answers based on the metrics that we will discuss below. In the second approach, we selected three questions that developers have struggled with in their development career and generated answers for those questions using GPT-3.5, GPT-4 and StackRAG. The developers were again asked to evaluate the answers from all models based on the same metrics. 
The three challenges are 
\textit{`How to do horizontal scaling of web sockets?'}, 
\textit{`How to import from a parent directory in Python?'}, and
\textit{`How to use function calling in openAI API?'}.

\subsection{Evaluation Metrics}
We used four different evaluation metrics to assess the performance of our model. Each of the metrics has a score between $1$ to $5$, one being the worst and 5 indicating the best. 

\textbf{Correctness (C)}: Is the response provided to the question correct?

\textbf{Accuracy (A)}: Does the response explain the solution of the asked question accurately?

\textbf{Relevance (R)}: Is the generated text related to the asked question in terms of the topic?

\textbf{Usefulness (U)}: Does the response provide information that is useful to solve the asked question?


% 1. How to do horizontal scaling of web sockets?
% 2. How to import from a parent directory in python?
% 3. How to use function calling in openAI API?

\subsection{Results}

Table~\ref{tab:usage} represents the average scores for the four metrics given by developers when the developers' usage of StackRAG throughout a full working day. 
As we can see, developers were mostly satisfied with the generated answers by StackRAG and found them useful for solving challenges they faced during development.

\begin{table}[h!]
  \centering
  \begin{tabular}{|c|c|c|c|c|}
    \hline
   \textbf{ Metric} & \textbf{C} &\textbf{ A}  & \textbf{R}  & \textbf{U}\\
    \hline
   \textbf{Average Score }& 4.33 &  4.33 & 4.33 & 4 \\
    \hline
  \end{tabular}
  \caption{Evaluation of StackRAG based on developers' usage in daily tasks. The scores are average of the developers' responses.}
  \label{tab:usage}
\end{table}



 \begin{table}[h!]
  \centering
  \begin{tabular}{|c|c|c|c|c|}
    \hline
    \textbf{Metric/Model} & \textbf{C} & \textbf{A}  & \textbf{R}  & \textbf{U}\\
    \hline
    \textbf{StackRAG} & 4.66 &  4.55 & 4.55 & 4.55 \\
    \hline
    \textbf{GPT-3.5} & 4.22 &  4.11 & 4 & 3.77 \\
    \hline
    \textbf{GPT-4} & 4.22 &  4.11 & 4.22 & 4.11 \\
    \hline
  \end{tabular}
  \caption{Evaluation of StackRAG and GPT models based on the selected questions.}
  \label{tab:comparison-gpt}
\end{table}

% \begin{table}[h!]
%   \centering
%   \begin{tabular}{|c|c|c|c|c|}
%     \hline
%     \textbf{Metric/Model} & \textbf{C} & \textbf{A}  & \textbf{R}  & \textbf{U}\\
%     \hline
%     \textbf{StackRAG} & 4.22 &  4.11 & 4.55 & 4.55 \\
%     \hline
%     \textbf{GPT-3.5} & 4.22 &  4.11 & 4 & 3.77 \\
%     \hline
%     \textbf{GPT-4} & 4.22 &  4.11 & 4.22 & 4.11 \\
%     \hline
%   \end{tabular}
%   \caption{Evaluation of StackRAG and GPT models based on the selected questions.}
%   \label{tab:comparison-gpt}
% \end{table}

Table~\ref{tab:comparison-gpt} shows the evaluation of StackRAG in comparison with GPT-3.5, GPT-4 models.
The result are the average scores given by the developers, where the developers scored the generated answers of the models for the pre-defined questions.
Even though StackRAG uses \FHF{GPT???} as the base model, it performs better than the two other models in all four metrics.  
This indicates that the developers find the answers generated by StackRAG more relevant to the topic and they found more useful information in the responses, in addition to being correct and accurate answers. 
When we discussed with the developers, they valued the provided links in the generated response.

\label{sec:bibtex}


==> notes.tex <==
Rise application title:
StackRAG tool to combine generative AI with SO knowledge


In my opinion they might still continue to use ChatGPT mainly because of the fact that it takes a lot more time for StackRAG to generate an answer compared to chatGPT. Also there are certain cases where it might not give an answer if there is no answer available in stackOverflow. I can handle that by making GPT answer a question based on its knowledge if there is no information available in StackOverflow, however, the problem of time will still remain. Nonetheless, if the goal of the user is the reliability and the relevance of the generated answer, than our tool is very likely to outperform other models because of the answers being grounded by information in SO.

Here is the link to my github repo: https://github.com/DavidAbrahamyan/AccurAnswer
Here is the link to overleaf: https://www.overleaf.com/project/66071e8b6b972bfb00229b89


Google forms:

https://docs.google.com/forms/d/1Fo0rvBB4T2W_5D8hMIqTd5qhuGFXe9qoQMhegfxrJ2E/edit?ts=66465734&exids=71471476,71471470

https://docs.google.com/forms/d/1PUjaJv_Ts2oS73TeWtexc0sXSEjLrYr2YAKf2BvWyvU/edit?ts=6646575f&exids=71471476,71471470

https://docs.google.com/forms/d/1f6XIvkVCh9It44chGTxrUs8vW-txp5W9X_Z_zrDZi48/edit?ts=66465758&exids=71471476,71471470

Hi Davit, 

See this: 
https://arxiv.org/pdf/2402.08801

Read RQ3 results and discussions. 
This is a good support for your work. 

For the evaluation, can you choose the topics they mention LLMs cannot answer, and choose some questions in each of those topics? 
Let me know how many topics there are. 
IF their dataset is available, we can choose the questions and topics as mentioned in the paper and just ask the models including yours to generate the results.
Let me know if their dataset and questions are open source.

We can then ask our students to evaluate the results and add to your Paper.

FHF


https://openai.com/index/api-partnership-with-stack-overflow/

AccrAnswer Link:
https://github.com/DavidAbrahamyan/AccurAnswer

